Engineering the sensitivity of macroscopic physical systems to variations in the fine-structure constant

Experiments aimed at searching for variations in the fine-structure constant $\alpha$ are based on spectroscopy of transitions in microscopic bound systems, such as atoms and ions, or resonances in optical cavities. The sensitivities of these systems to variations in $\alpha$ are typically on the order of unity and are fixed for a given system. For heavy atoms, highly charged ions and nuclear transitions, the sensitivity can be increased by benefiting from the relativistic effects and favorable arrangement of quantum states. This article proposes a new method for controlling the sensitivity factor of macroscopic physical systems. Specific concepts of optical cavities with tunable sensitivity to $\alpha$ are described. These systems show qualitatively different properties from those of previous studies of the sensitivity of macroscopic systems to variations in $\alpha$, in which the sensitivity was found to be fixed and fundamentally limited to an order of unity. Although possible experimental constraints attainable with the specific optical cavity arrangements proposed in this article do not yet exceed the present best constraints on $\alpha$ variations, this work paves the way for developing new approaches to searching for variations in the fundamental constants of physics.

==> bibliography.tex <==

@article{Jansen2011,
  title = {Methanol as a Sensitive Probe for Spatial and Temporal Variations of the Proton-to-Electron Mass Ratio},
  author = {Jansen, P and Xu, LH and Kleiner, I and Ubachs, W and Bethlem, HL},
  journal = {Phys. Rev. Lett.},
  volume = {106},
  issue = {10},
  pages = {100801},
  numpages = {4},
  year = {2011},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.106.100801},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.100801}
}

@article{fadeev2020sensitivity,
  title={Sensitivity of $^{229}$\uppercase{T}h nuclear clock transition to variation of the fine-structure constant},
  author={Fadeev, P and Berengut, JC and Flambaum, VV},
  journal={Phys. Rev. A},
  volume={102},
  number={5},
  pages={052833},
  year={2020},
  publisher={APS}
}


@article{wcislo2018first,
	author = {Wcis{\l}o, P and Ablewski, P and Beloy, K and Bilicki, S and Bober, M and Brown, R and Fasano, R and Ciury{\l}o, R and Hachisu, H and Ido, T and Lodewyck, J and Ludlow, A and McGrew, W and Morzy{\'n}ski, P and Nicolodi, D and Schioppo, M and Sekido, M and Le Targat, R and Wolf, P and Zhang, X and Zjawin, B and Zawada, M},
	title = {New bounds on dark matter coupling from a global network of optical atomic clocks},
	 journal={Sci. Adv.},
    volume = {4},
	number = {12},
	pages= {eaau4869},
	year = {2018},
	publisher = {American Association for the Advancement of Science},
	
}


@article{arvanitaki2015searching,
  title={Searching for dilaton dark matter with atomic clocks},
  author={Arvanitaki, A and Huang, J and Van Tilburg, K},
  journal={Phys. Rev. D},
  volume={91},
  number={1},
  pages={015015},
  year={2015},
  publisher={APS}
}

@article{kozlov2018sensitivity,
author = {Kozlov, MG and Budker, D},
title = {Comment on Sensitivity Coefficients to Variation of Fundamental Constants},
journal = {Annalen der Physik},
pages = {1800254},
year={2018}
}

@article{kozlov2018sensitivity-app,
author = {Kozlov, MG and Budker, D},
title = {Comment on Sensitivity Coefficients to Variation of Fundamental Constants},
journal = {Annalen der Physik},
pages = {1800254},
year={2018}
}

@article{angstmann2006narrow,
  title={Narrow atomic transitions with enhanced sensitivity to variation of the fine structure constant},
  author={Angstmann, EJ and Dzuba, VA and Flambaum, VV and Nevsky, A Yu and Karshenboim, Savely G},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={39},
  number={8},
  pages={1937},
  year={2006},
  publisher={IOP Publishing}
}




@incollection{barrow2003constants,
  title={Constants and variations: from alpha to omega},
  author={Barrow, JD},
  booktitle={The Cosmology of Extra Dimensions and Varying Fundamental Constants},
  pages={207},
  year={2003},
  publisher={Springer}
}


@article{pavsteka2018material,
  title={Material Size Dependence on Fundamental Constants},
  author={Pa{\v{s}}teka, LF and Hao, Y and Borschevsky, A and Flambaum, VV and Schwerdtfeger, P},
  journal={Phys. Rev. Lett.},
  volume={122},
  number={16},
  pages={160801},
  year={2019},
  publisher={APS}
}

@article{ushijima2015cryogenic,
  title={Cryogenic optical lattice clocks},
  author={Ushijima, I and Takamoto, M and Das, M and Ohkubo, T and Katori, H},
  journal={Nat. Photon.},
  volume={9},
  number={3},
  pages={185},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{berengut2010enhanced,
  title={Enhanced laboratory sensitivity to variation of the fine-structure constant using highly charged ions},
  author={Berengut, JC and Dzuba, VA and Flambaum, VV},
  journal={Phys. Rev. Lett.},
  volume={105},
  number={12},
  pages={120801},
  year={2010},
  publisher={APS}
}

@article{hansch,
  title={Nobel Lecture: Passion for precision},
  author={H{\"a}nsch, TW},
  journal={Rev. Mod. Phys.},
  volume={78},
  pages={1297},
  year={2006},
}


@article{dzuba2015optical,
  title={Optical clock sensitive to variations of the fine-structure constant based on the \uppercase{H}o$^{14+}$ ion},
  author={Dzuba, VA and Flambaum, VV and Katori, H},
  journal={Phys. Rev. A},
  volume={91},
  number={2},
  pages={022119},
  year={2015},
  publisher={APS}
}

@article{dzuba2015actinide,
  title={Actinide ions for testing the spatial $\alpha$-variation hypothesis},
  author={Dzuba, VA and Safronova, MS and Safronova, UI and Flambaum, VV},
  journal={Phys. Rev. A},
  volume={92},
  number={6},
  pages={060502},
  year={2015},
  publisher={APS}
}

@article{huntemann2014improved,
  title={Improved limit on a temporal variation of $m_p/m_e$ from comparisons of \uppercase{Y}b$^{+}$ and \uppercase{C}s atomic clocks},
  author={Huntemann, N and Lipphardt, B and Tamm, Chr and Gerginov, V and Weyers, S and Peik, E},
  journal={Phys. Rev. Lett.},
  volume={113},
  number={21},
  pages={210802},
  year={2014},
  publisher={APS}
}

@article{hees2016searching,
  title={Searching for an oscillating massive scalar field as a dark matter candidate using atomic hyperfine frequency comparisons},
  author={Hees, A and Gu{\'e}na, J and Abgrall, M and Bize, S and Wolf, P},
  journal={Phys. Rev. Lett.},
  volume={117},
  number={6},
  pages={061301},
  year={2016},
  publisher={APS}
}

@article{van2015search,
  title={Search for ultralight scalar dark matter with atomic spectroscopy},
  author={Van Tilburg, K and Leefer, N and Bougas, L and Budker, D},
  journal={Phys. Rev. Lett.},
  volume={115},
  number={1},
  pages={011802},
  year={2015},
  publisher={APS}
}



@article{aoyama2012tenth,
  title={Tenth-order \uppercase{QED} contribution to the electron g-2 and an improved value of the fine structure constant},
  author={Aoyama, T and Hayakawa, M and Kinoshita, T and Nio, M},
  journal={Phys. Rev. Lett.},
  volume={109},
  number={11},
  pages={111807},
  year={2012},
  publisher={APS}
}

@article{zhang2017ultrastable,
  title={Ultrastable Silicon Cavity in a Continuously Operating Closed-Cycle Cryostat at 4 \uppercase{K}},
  author={Zhang, W and Robinson, JM and Sonderhouse, L and Oelker, E and Benko, C and Hall, JL and Legero, T and Matei, DG and Riehle, F and Sterr, U and others},
  journal={Phys. Rev. Lett.},
  volume={119},
  number={24},
  pages={243601},
  year={2017},
  publisher={APS}
}

@article{safronova2018two,
  title={Two clock transitions in neutral \uppercase{Y}b for the highest sensitivity to variations of the fine-structure constant},
  author={Safronova, MS and Porsev, SG and Sanner, Chr and Ye, J},
  journal={Phys. Rev. Lett.},
  volume={120},
  number={17},
  pages={173001},
  year={2018},
  publisher={APS}
}


@article{litvinova2009nuclear,
  title={Nuclear structure of lowest $^{229}$\uppercase{T}h states and time-dependent fundamental constants},
  author={Litvinova, E and Feldmeier, H and Dobaczewski, J and Flambaum, V},
  journal={Phys. Rev. C},
  volume={79},
  number={6},
  pages={064303},
  year={2009},
  publisher={APS}
}

@article{safronova2018nuclear,
  title={Nuclear charge radii of $^{229}$\uppercase{T}h from isotope and isomer shifts},
  author={Safronova, MS and Porsev, SG and Kozlov, MG and Thielking, J and Okhapkin, MV and G{\l}owacki, P and Meier, DM and Peik, E},
  journal={arXiv preprint arXiv:1806.03525},
  year={2018}
}

@article{bagdonaite2012stringent,
  title={A stringent limit on a drifting proton-to-electron mass ratio from alcohol in the early universe},
  author={Bagdonaite, J and Jansen, P and Henkel, Chr and Bethlem, HL and Menten, KM and Ubachs, W},
  journal={Science},
  pages={46},
  volume={339},
  year={2013},
  publisher={American Association for the Advancement of Science}
}

@article{berengut2012optical,
  title={Optical transitions in highly charged californium ions with high sensitivity to variation of the fine-structure constant},
  author={Berengut, JC and Dzuba, VA and Flambaum, VV and Ong, A},
  journal={Phys. Rev. Lett.},
  volume={109},
  number={7},
  pages={070802},
  year={2012},
  publisher={APS}
}

@article{wcislo2016searching,
  title={Searching for topological defect dark matter with optical atomic clocks},
  author={Wcislo, P and Morzynski, P and Bober, M and Cygan, A and Lisak, D and Ciurylo, R and Zawada, M},
  journal={Nat. Astro.},
  year={2016},
  pages={0009},
  volume={1}
}

@article{rosenband2008frequency,
  title={Frequency ratio of \uppercase{A}l$^{+}$ and \uppercase{H}g$^{+}$ single-ion optical clocks; metrology at the 17th decimal place},
  author={Rosenband, T and Hume, DB and Schmidt, PO and Chou, CW and Brusch, A and Lorini, L and Oskay, WH and Drullinger, RE and Fortier, TM and Stalnaker, JE and others},
  journal={Science},
  volume={319},
  number={5871},
  pages={1808--1812},
  year={2008},
  publisher={American Association for the Advancement of Science}
}

@article{godun2014frequency,
  title={Frequency Ratio of Two Optical Clock Transitions in $^{171 }$\uppercase{Y}b$^{+}$ and Constraints on the Time Variation of Fundamental Constants},
  author={Godun, RM and Nisbet-Jones, PBR and Jones, JM and King, SA and Johnson, LAM and Margolis, HS and Szymaniec, K and Lea, SN and Bongs, K and Gill, P},
  journal={Phys. Rev. Lett.},
  volume={113},
  number={21},
  pages={210801},
  year={2014},
  publisher={APS}
}

@article{stadnik2016enhanced,
  title={Enhanced effects of variation of the fundamental constants in laser interferometers and application to dark-matter detection},
  author={Stadnik, YV and Flambaum, VV},
  journal={Phys. Rev. A},
  volume={93},
  number={6},
  pages={063630},
  year={2016},
  publisher={APS}
}



@article{flambaum2009search,
  title={Search for variation of the fundamental constants in atomic, molecular, and nuclear spectra},
  author={Flambaum, VV and Dzuba, VA},
  journal={Can J Phys.},
  volume={87},
  number={1},
  pages={25--33},
  year={2009},
  publisher={NRC Research Press}
}

@article{pavsteka2015search,
  title={Search for the variation of fundamental constants: Strong enhancements in X $\Pi$ 2 cations of dihalogens and hydrogen halides},
  author={Pa{\v{s}}teka, LF and Borschevsky, A and Flambaum, VV and Schwerdtfeger, P},
  journal={Phys. Rev. A},
  volume={92},
  number={1},
  pages={012103},
  year={2015},
  publisher={APS}
}

@article{stadnik2015searching,
  title={Searching for dark matter and variation of fundamental constants with laser and maser interferometry},
  author={Stadnik, YV and Flambaum, VV},
  journal={Phys. Rev. Lett.},
  volume={114},
  number={16},
  pages={161301},
  year={2015},
  publisher={APS}
}

@article{fischer2004new,
  title={New limits on the drift of fundamental constants from laboratory measurements},
  author={Fischer, M and Kolachevsky, N and Zimmermann, M and Holzwarth, R and Udem, Th and H{\"a}nsch, TW and Abgrall, M and Gr{\"u}nert, J and Maksimovic, I and Bize, S and others},
  journal={Phys. Rev. Lett.},
  volume={92},
  number={23},
  pages={230802},
  year={2004},
  publisher={APS}
}

@article{derevianko2014hunting,
  title={Hunting for topological dark matter with atomic clocks},
  author={Derevianko, A and Pospelov, M},
  journal={Nat. Phys.},
  volume={10},
  number={12},
  pages={933--936},
  year={2014},
  publisher={Nature Research}
}

@article{flambaum2006enhancedmole,
  title={Enhanced effect of temporal variation of the fine-structure constant in diatomic molecules},
  author={Flambaum, VV},
  journal={Phys. Rev. A},
  volume={73},
  number={3},
  pages={034101},
  year={2006},
  publisher={APS}
}

@article{flambaum2006enhancednuclear,
  title={Enhanced Effect of Temporal Variation of the Fine Structure Constant and the Strong Interaction in $^{229}$\uppercase{T}h},
  author={Flambaum, VV},
  journal={Phys. Rev. Lett.},
  volume={97},
  number={9},
  pages={092502},
  year={2006},
  publisher={APS}
}

@article{leibrandt2011field,
  title={Field-test of a robust, portable, frequency-stable laser},
  author={Leibrandt, DR and Thorpe, MJ and Bergquist, JC and Rosenband, T},
  journal={Opt. Express},
  volume={19},
  number={11},
  pages={10278},
  year={2011},
  publisher={Optical Society of America}
}

@article{leibrandt2013cavity,
  title={Cavity-stabilized laser with acceleration sensitivity below $10^{-12} g^{-1}$},
  author={Leibrandt, DR and Bergquist, JC and Rosenband, T},
  journal={Phys. Rev. A},
  volume={87},
  number={2},
  pages={023829},
  year={2013},
  publisher={APS}
}

@article{savalle2019novel,
  title={Novel approaches to dark-matter detection using space-time separated clocks},
  author={Savalle, E and Roberts, BM and Frank, F and Pottie, PE and McAllister, BT and Dailey, CB and Derevianko, A and Wolf, P},
  journal={arXiv preprint arXiv:1902.07192},
  year={2019}
}

@article{matei20171,
    title={1.5 $\mu$m Lasers with Sub-10 m\uppercase{H}z Linewidth},
  author={Matei, DG and Legero, T and H{\"a}fner, S and Grebing, Ch and Weyrich, R and Zhang, W and Sonderhouse, L and Robinson, JM and Ye, J and Riehle, F and others},
  journal={Phys. Rev. Lett.},
  volume={118},
  number={26},
  pages={263202},
  year={2017},
  publisher={APS}
}

@article{robinson2019crystalline,
  title={Crystalline optical cavity at 4 \uppercase{K} with thermal-noise-limited instability and ultralow drift},
  author={Robinson, JM and Oelker, E and Milner, WR and Zhang, W and Legero, T and Matei, DG and Riehle, F and Sterr, U and Ye, J},
  journal={Optica},
  volume={6},
  number={2},
  pages={240},
  year={2019},
  publisher={Optical Society of America}
}

@article{uzan2003fundamental,
  title={The fundamental constants and their variation: observational and theoretical status},
  author={Uzan, JP},
  journal={Rev. Mod. Phys.},
  volume={75},
  number={2},
  pages={403},
  year={2003}
}

@article{lammerzahl2006search,
  title={The search for quantum gravity effects II: Specific predictions},
  author={L{\"a}mmerzahl, C},
  journal={Applied Physics B},
  volume={84},
  number={4},
  pages={563},
  year={2006},
  publisher={Springer}
}

@article{robinson2021thermal,
  title={Thermal noise and mechanical loss of {S}i{O}$_2$/{T}a$_2${O}$_5$ optical coatings at cryogenic temperatures},
  author={Robinson, JM and Oelker, E and Milner, WR and Kedar, D and Zhang, W and Legero, T and Matei, DG and H{\"a}fner, S and Riehle, F and Sterr, U and others},
  journal={Optics Letters},
  volume={46},
  number={3},
  pages={592},
  year={2021},
  publisher={Optical Society of America}
}

@article{leefer2013new,
  title={New limits on variation of the fine-structure constant using atomic dysprosium},
  author={Leefer, N and Weber, CTM and Cing{\"o}z, A and Torgerson, JR and Budker, D},
  journal={Phys. Rev. Lett.},
  volume={111},
  number={6},
  pages={060801},
  year={2013},
  publisher={APS}
}

@article{flambaum2007enhanced,
  title={Enhanced sensitivity to the time variation of the fine-structure constant and m p/m e in diatomic molecules},
  author={Flambaum, VV and Kozlov, MG},
  journal={Physical review letters},
  volume={99},
  number={15},
  pages={150801},
  year={2007},
  publisher={APS}
}

@article{flambaum2006enhancedmol,
  title={Enhanced effect of temporal variation of the fine-structure constant in diatomic molecules},
  author={Flambaum, VV},
  journal={Physical Review A},
  volume={73},
  number={3},
  pages={034101},
  year={2006},
  publisher={APS}
}

@article{dzuba1999calculations,
  title={Calculations of the relativistic effects in many-electron atoms and space-time variation of fundamental constants},
  author={Dzuba, VA and Flambaum, VV and Webb, JK},
  journal={Physical Review A},
  volume={59},
  number={1},
  pages={230},
  year={1999},
  publisher={APS}
}

@article{dzuba1999space,
  title={Space-time variation of physical constants and relativistic corrections in atoms},
  author={Dzuba, VA and Flambaum, VV and Webb, JK},
  journal={Physical Review Letters},
  volume={82},
  number={5},
  pages={888},
  year={1999},
  publisher={APS}
}
